A Second-Order Reachable Sets Computation Scheme via a Cauchy-Type Variational Hamilton-Jacobi-Isaacs Equation

Motivated by the scalability limitations of Eulerian methods for variational Hamilton-Jacobi-Isaacs (HJI) formulations that provide a least restrictive controller in problems that involve state or input constraints under a worst-possible disturbance, we introduce a second-order, successive sweep algorithm for computing the zero sublevel sets of a popular reachability value functional. Under sufficient HJI partial differential equation regularity and continuity assumption throughout the state space, we show that with state feedback control under the worst-possible disturbance, we can compute the state set that are reachable within a prescribed verification time bound.

==> sections/related.tex <==
\section{Background}
\label{sec:back}

Suppose that there exists a vector field, $\hamfunc: \left[t_i, t_f\right] \times \bb{R}^m \times \bb{R}^m \rightarrow \bb{R}$ that is continuous, and $g: \bb{R}^m\rightarrow \bb{R}^m$ is bounded and uniformly continuous, a bounded and uniformly continuous function $\valuefunc: \left[t_i, t_f\right] \times \bb{R}^m \rightarrow \bb{R}^m$ is a solution of the following Hamilton-Jacobi partial differential equation
%
\begin{align}
	\dfrac{\partial \valuefunc}{\partial t} + \hamfunc(t, \state, D\valuefunc) &= 0 \quad \text{ in } \left[t_i, t_f\right] \times \bb{R}^n \\
	\valuefunc(t_i, \state) &= g(\state)   \quad \text{ in } \bb{R}^n
	\label{eq:hj_pde}
\end{align}
%
provided \eqref{eq:hj_pde} holds. $\valuefunc(\state, t)$ admits an expansion as standard cost-to-go integral plus the terminal cost, particular to Isaac's construction. In reachability analysis, we discard the cost-to-go and concentrate on solving the terminal cost functional.

%\paragraph{Dynamic Programming and Two-Person Games}
%The formal relationships between the dynamic programming (DP) optimality condition for the \textit{value} in differential two-person zero-sum games, and the solutions to PDEs that solve ``min-max" or ``max-min" type nonlinearity (the Isaacs' equation) was presented in~\cite{Isaacs1965}. 
%If the \textit{value} functions are smooth enough, then they solve certain first-order partial differential equations (PDE) problems with  ``max-min" or ``min-max"-type nonlinearity.  However, the DP value functions are seldom regular enough to admit a solution in the classical sense.  
%``Weaker" solutions on the other hand~\cite{Lions1982, Evans1984, Crandall1984, CrandallLaxFriedrichs, Souganidis} provide generalized ``viscosity" solutions to HJ PDEs under relaxed regularity conditions; these viscosity solutions are not necessarily differentiable anywhere in the state space, and the only regularity prerequisite in the definition is continuity~\cite{Crandall1983viscosity}. 
%However, wherever they are differentiable, they satisfy the  upper and lower values of HJ PDEs in a classical sense. 
%Thus, they lend themselves well to many real-world problems existing at the interface of discrete, continuous, and hybrid systems~\cite{LygerosReachability, OsherFronts, Mitchell2020, Souganidis, Mitchell2005}. 
%Viscosity Solutions to \textit{Cauchy-type} HJ Equations admit usefulness in backward reachability analysis~\cite{Mitchell2005}. 
%In scope and focus, this is the bulwark upon which we build our formulation in this paper.


\paragraph{Reachability for Systems Verification.}
Reachability analysis is concerned with finding the set forward (respectively backward) states that are reachable from a set of initial (resp. target) state sets, within a given a time bound. As opposed to reachability analysis for safety verification in software model checking\footnote{Here, a program $P$ with a specific property, $\Pi$, is said to be safe if every computation of $P$ is in $\Pi$ and returns ``unsafe" in the contrary case~\cite{jhala2009software}.} where single program runs are computed per time from an initial state to verify safety, with reachability analysis every possible trajectory or execution of a system are computed from all possible initial (resp. terminal states) states. This verification problem usually consists in finding a \textit{reachable states set} that lie along the trajectory of the solution to a first order nonlinear partial differential equation that originates from some initial state $\state_0 = \state(0)$ up to a specified time bound, $t=t_f$. 
%Reachability could be analyzed in a 
%%
%\begin{inparaenum}[(i)]
%	\item \textit{forward} sense, whereupon system trajectories are examined to determine if they enter certain states from an \textit{initial set};
%	%
%	\item \textit{backward} sense, whereupon system trajectories are examined to determine if they enter certain \textit{target sets};
%	%
%	\item \textit{reach set} sense, in which they are examined to see if states reach a set at a \textit{particular time}; or
%	%
%	\item \textit{reach tube} sense, in which they are evaluated that they reach a set at a point \textit{during a time interval}.	
%\end{inparaenum} 

Backward reachable sets (BRS) or tubes (BRTs) are popularly analyzed as a game of two vehicles with non-stochastic dynamics~\cite{Merz1972}. 
Such BRTs possess discontinuity at cross-over points (which exist at edges) on the surface of the  tube, and are usually be non-convex~\cite{Molux2022WAFR, Mitchell2005, DecompChenHerbert}. 
%Therefore, treating the end-point constraints under these discontinuity characterizations need careful consideration and analysis when switching control laws if the underlying PDE does not have continuous partial  derivatives \todo{(we discuss this further in \autoref{sec:methods})}. 

Instead of using state space discretization methods and employing Lax-Friedrichs schemes to resolve the value function   over a global mesh, we resolve to classical successive sweep optimal control algorithms~\cite{Mitter1966, McReynolds1967}, in particular a differential dynamic programming (DDP)~\cite{Mayne1966, Jacobson1968new, JacobsonMayne}  variant~\cite{iDG}, which are iterative algorithms for obtaining solutions to optimal control problems. Similar to the monotone  characteristics of~\cite{CrandallLaxFriedrichs, CrandallFractional}, these methods (under appropriate conditions~\cite{iDG}) assure a monotone solution on the state space.

%Henceforward, for ease of readability, we will remove the minus superscript on the lower value and Hamiltonian. The value function is the viscosity solution to this HJ PDE \cite{Souganidis}. 
%Note that this PDE must be applied at every grid point in the state space and at every instant of time within the time horizon. As the system scales in dimension, this computation scales exponentially.

Once computed, the value function provides a safety certificate (defined by its zero level set) and corresponding safety controller (defined by the spatial gradients along the zero level set). \shnote{don't know if we should go into the online control portion of this or not}

%In addition to producing a value function, the dynamic programming process can be used to generate and minimum time-to-reach (TTR) function. This is a function that maps initial conditions to the minimum time horizon required to reach the target set.  This can be computed by ``stacking'' the zero level sets of the value function as it propagates backwards in time~\cite{Mitchell2020, BasarBook, AthansFalb}. \shnote{cite Ian Mitchell, maybe Insoon;} 

%\paragraph{Global Mesh-based Methods and Up-Scaling Reachability Analysis}
%Consider a reachability problem defined in a space of dimension $D=12$ based on the non-incremental time-space discretization of each space coordinate. For $N=100$ nodes, the total nodes required is $10^{120}$ on the volumetric grid\footnote{Whereas, there are only $10^{97}$ baryons in the observable universe (excluding dark matter)!}. The curse of dimensionality~\cite{Bellman1957} greatly incapacitates current uniform grid discretization methods for guaranteeing the robustness of backward reachable sets (BRS) and tubes (BRTs)~\cite{Mitchell2005} of complex systems. 
%Recent works have started exploring scaling up the Cauchy-type HJ problem for guaranteeing safety of higher-dimensional physical systems: the authors of~\cite{Bajcsy} provide local updates to BRS in  unknown static environments with obstacles that may be unknown \textit{a priori} to the agent; using standard meshing techniques for time-space uniform discretization over the entire physical space, and only updating points traversed locally, a safe navigation problem was solved in an environment assumed to be static. 
%This makes it non-amenable to \textit{a priori} unknown \textit{dynamic} environments where the optimal value to the min-max HJ problem may need to be adaptively updated based on changing dynamics. 
%
%In ~\cite{SylviaScalability}, the grid was naively refined along the temporal dimension, leveraging local decomposition schemes together with warm-starting optimization of the value function from previous solutions in order to accelerate learning for safety under the assumption that the system is either completely decoupled, or coupled over so-called ``self-contained subsystems".  While the empirical results of~\cite{Bansal} demonstrate the feasibility of optimizing for the optimal value function in backward reachability analysis for up to ten dimensions for a system of Dubins vehicles, there are no guarantees that are provided. An analysis exists for a 12 dimensional systems~\cite{KaynamaScalable} with up to a billion data points in the state space, that generates robustly optimal trajectories. However, this is restricted to {linear systems}. Other associated techniques scale reachability with function approximators~\cite{FisacTAC, FisacICRA} in a reinforcement learning framework; again these methods lose the hard safety guarantees owing to the approximation in value function space.  
%

